Global Sensitivity Analysis and Estimation of Model Error, Toward Uncertainty Quantification in Scramjet Computations

The development of scramjet engines is an important research area for advancing hypersonic and orbital flights. Progress toward optimal engine designs requires accurate flow simulations together with uncertainty quantification. However, performing uncertainty quantification for scramjet simulations is challenging due to the large number of uncertain parameters involved and the high computational cost of flow simulations. These difficulties are addressed in this paper by developing practical uncertainty quantification algorithms and computational methods, and deploying them in the current study to large-eddy simulations of a jet in crossflow inside a simplified HIFiRE Direct Connect Rig scramjet combustor. First, global sensitivity analysis is conducted to identify influential uncertain input parameters, which can help reduce the systems stochastic dimension. Second, because models of different fidelity are used in the overall uncertainty quantification assessment, a framework for quantifying and propagating the uncertainty due to model error is presented. These methods are demonstrated on a nonreacting jet-in-crossflow test problem in a simplified scramjet geometry, with parameter space up to 24 dimensions, using static and dynamic treatments of the turbulence subgrid model, and with two-dimensional and three-dimensional geometries.

==> Makefile <==
SECTIONS = $(wildcard sections/*.tex)
FIGURES_TIKZ = $(shell find figures -type f -name '*.tikz')
FIGURES_TIKZ_PDF = $(FIGURES_TIKZ:%.tikz=%.pdf)
FIGURES_EPS = $(shell find figures -type f -name '*.eps')
FIGURES_EPS_PDF = $(FIGURES_EPS:%.eps=%-eps-converted-to.pdf)
FIGURES_ONLY_PDF = $(shell find figures -type f -name '*.pdf')

all: main.pdf

main.pdf: main.tex $(SECTIONS) $(FIGURES_TIKZ_PDF) $(FIGURES_EPS) \
	$(FIGURES_ONLY_PDF) newcommands_all.tex local.bib
	latexmk -pdf -interaction=nonstopmode main.tex

$(FIGURES_TIKZ_PDF): %.pdf: %.tikz figures/header figures/footer
	cat figures/header $< figures/footer > figures/temp.tex;
	latexmk -pdf -interaction=nonstopmode -jobname=$(basename $@) figures/temp.tex

.PHONY: clean cleanmain cleanall

# You can choose which renegerable files you want to add or exclude below.
clean:
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.glo *.idx *.ilg *.ind *.lof *.log *.lot \
	      *.nav *.out *.ps *.snm *.spl *.toc
	@echo -n "Start cleaning tikz regenerable files..."
	@rm -f $(FIGURES_TIKZ:%.tikz=%.aux)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.bbl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.blg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.brf)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.dvi)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fdb_latexmk)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fls)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.glo)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.idx)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ilg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ind)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lof)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.log)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lot)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.nav)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.out)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ps)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.snm)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.spl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.toc)
	@echo "done."
	cd figures; rm -f temp.tex ;\
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.idx *.ilg *.ind *.log *.out *.ps *.spl *.toc

cleanmain:
	@make clean
	rm -f main.pdf

cleanall:
	@make cleanmain
	@echo "Start cleaning tikz pdf files..."
	@rm -f $(FIGURES_TIKZ_PDF)
	@echo "done."
	@echo "Start cleaning eps pdf files..."
	@rm -f $(FIGURES_EPS_PDF)
	@echo "done."

